PyQMC: an all-Python real-space quantum Monte Carlo module in PySCF

We describe a new open-source Python-based package for high accuracy correlated electron calculations using quantum Monte Carlo (QMC) in real space: PyQMC. PyQMC implements modern versions of QMC algorithms in an accessible format, enabling algorithmic development and easy implementation of complex workflows. Tight integration with the PySCF environment allows for simple comparison between QMC calculations and other many-body wave function techniques, as well as access to high accuracy trial wave functions.

==> fig_flowchart_user_vmc.tex <==
\begin{tikzpicture}[>=stealth, box/.style={rounded corners=3mm, draw, fill=green!10!white}]

\node(output) [box, minimum width=4cm, minimum height=1cm]{\parbox{4cm}{\centering Output observables}};

\node(acc) [box, above left=4.5cm and 5mm of output.north, anchor=east, minimum width=3cm, minimum height=1cm]{\centering Accumulators};

\node(wf) [box, above right=4.5cm and 5mm of output.north, anchor=west, minimum width=2cm, minimum height=1cm]{\centering Wave functions};

\node(pyqmcvmc) [box, above left=12mm and 20mm of output.north, anchor=south, minimum width=28mm, minimum height=1.5cm]{\parbox{2.2cm}{\centering PyQMC VMC}};
\node(uservmc) [box, above right=12mm and 20mm of output.north, anchor=south, minimum width=28mm, minimum height=1.5cm]{\parbox{2.2cm}{\centering User-defined VMC}};

\draw[->] (acc.south) -- (pyqmcvmc);
\draw[->] (acc.south) -- (uservmc);
\draw[->] (wf.south) -- (pyqmcvmc);
\draw[->] (wf.south) -- (uservmc);
\draw[->] (pyqmcvmc) -- (output);
\draw[->] (uservmc) -- (output);
\end{tikzpicture}

